High-Resolution Depth Estimation for 360-degree Panoramas through Perspective and Panoramic Depth Images Registration

We propose a novel approach to compute high-resolution (2048x1024 and higher) depths for panoramas that is significantly faster and qualitatively and qualitatively more accurate than the current state-of-the-art method (360MonoDepth). As traditional neural network-based methods have limitations in the output image sizes (up to 1024x512) due to GPU memory constraints, both 360MonoDepth and our method rely on stitching multiple perspective disparity or depth images to come out a unified panoramic depth map. However, to achieve globally consistent stitching, 360MonoDepth relied on solving extensive disparity map alignment and Poisson-based blending problems, leading to high computation time. Instead, we propose to use an existing panoramic depth map (computed in real-time by any panorama-based method) as the common target for the individual perspective depth maps to register to. This key idea made producing globally consistent stitching results from a straightforward task. Our experiments show that our method generates qualitatively better results than existing panorama-based methods, and further outperforms them quantitatively on datasets unseen by these methods.

==> rebuttal.tex <==
R1 Weaknesses:

- Given the additional information stream and runtime costs, one would expect the results compared to pure single-shot estimates to be much better, especially when the latter are simply upscaled.

- As indicated by the authors an advantage of such a method would be higher detail preservation, but this is only qualitatively assessed. It is also rather important as any edge misalignment would be accentuated by the Laplacians and thus the reconstruction/fusion, and thus, it should be an important quantitative experiment.

Justification
On one hand, the concept is novel and sound, its presentation is appropriate and is accompanied by lots of experiments and results. On the other hand, the relative performance to a bilinearly upsampled (x4 and x2) single-shot estimate is not the expected one. The latter is bound to have its performance deteriorated as linear upsampling blurs edges and does not respect equirectangular distortion. Further, one of the proposed techniques advantages (preservation of details), which can also be a significant weakness in the cases of edge misalignment, is only partly assessed.
Concluding, my recommendation currently reflects this mixed feeling and will be refined post-discussion.

R2 weaknesses:

- While the authors claim their method produces "high resolution", it only shows performance at 2K and 4K resolutions. It's better to show the performance at a higher resolution to show how high it can go.

- On Matterport3D (the training object of the panoramic depth estimation method), the optimized panoramic depth estimation performance actually degrades compared to the equipped panoramic depth estimation method. Better to discuss the root cause. Is it due to inconsistent performance of perspective and panoramic depth estimation methods, or due to the optimization design itself.

Justification
Overall, I don't think the paper is written in a way that does a good job of justifying the paper's position. I would view this paper as a flexible module that can be equipped with any perspective image depth estimation method and panorama depth estimation method to improve performance on new datasets, rather than datasets equipped with method training. Also, the claimed "high resolution" shows some preliminary experiments, but it's still not known how high the algorithm can go.
I do see some advantages to this paper, but the disadvantages are also obvious. So I vote for borderline.

R3 weaknesses:

-The method described in the article is overly complicated and I'm concerned if it's necessary. Since it is an improvement based on existing methods, why not use the method of image super-resolution (e.g., use the existing SOTA method to obtain a low-resolution depth map, and then apply super-resolution to the depth image)?
- The authors mention that their method is faster, but this method is incremental, which means that the inference speed of the method is likely limited by the method they use. So this statement is inaccurate.
- The method described is more complex and it might be easier to understand if there were more diagrams.
- Some important work was missed [A, B, C, D]. Similar to this paper, A proposes a more easier rotation-based projection strategy to achieve boundary consistency of projection perspectives. Based on tangent images, B propose PanoFormer and claim that it can apply to high resolution only by adding conv layers.

[A] Shen, Z., Lin, C., Nie, L., Liao, K., & Zhao, Y. (2021, July). Distortion-tolerant monocular depth estimation on omnidirectional images using dual-cubemap. In 2021 IEEE International Conference on Multimedia and Expo (ICME) (pp. 1-6). IEEE.

[B] Shen, Z., Lin, C., Liao, K., Nie, L., Zheng, Z., & Zhao, Y. (2022). PanoFormer: Panorama Transformer for Indoor 360 {\deg} Depth Estimation. In Proceedings of the European Conference on Computer Vision (ECCV)

[C] Eder, M., Price, T., Vu, T., Bapat, A. and Frahm, J.M., 2019. Mapped convolutions. arXiv preprint arXiv:1906.11096.

[D] Tateno, K., Navab, N. and Tombari, F., 2018. Distortion-aware convolutional filters for dense prediction in panoramic images. In Proceedings of the European Conference on Computer Vision (ECCV) (pp. 707-722).
